Tightening Bounds on Probabilities of Causation By Merging Datasets

Probabilities of Causation (PoC) play a fundamental role in decision-making in law, health care and public policy. Nevertheless, their point identification is challenging, requiring strong assumptions, in the absence of which only bounds can be derived. Existing work to further tighten these bounds by leveraging extra information either provides numerical bounds, symbolic bounds for fixed dimensionality, or requires access to multiple datasets that contain the same treatment and outcome variables. However, in many clinical, epidemiological and public policy applications, there exist external datasets that examine the effect of different treatments on the same outcome variable, or study the association between covariates and the outcome variable. These external datasets cannot be used in conjunction with the aforementioned bounds, since the former may entail different treatment assignment mechanisms, or even obey different causal structures. Here, we provide symbolic bounds on the PoC for this challenging scenario. We focus on combining either two randomized experiments studying different treatments, or a randomized experiment and an observational study, assuming causal sufficiency. Our symbolic bounds work for arbitrary dimensionality of covariates and treatment, and we discuss the conditions under which these bounds are tighter than existing bounds in literature. Finally, our bounds parameterize the difference in treatment assignment mechanism across datasets, allowing the mechanisms to vary across datasets while still allowing causal information to be transferred from the external dataset to the target dataset.

==> sections/causal-invariance.tex <==
%\documentclass[../main.tex]{subfiles}
%\begin{document}
To borrow causal information across different sources of data, we must first identify causal quantities that remain invariant across these different sources of data. The principle of independent mechanisms (see Principle 2.1 of \cite{peters2017elements}) allows to define such invariances across datasets.  
For example, consider the given SCM associated with the causal graph in Fig. X.
\begin{align*}
    X &\leftarrow f_X(u_X)\\
    Y &\leftarrow f_Y(u_Y)\\
    Z &\leftarrow f_Z(X, Y, u_Z)
\end{align*}
We assume $P(Z_{\textbf{x}, \textbf{y}})$ remains invariant across the two given marginals, i.e. the same mechanism $f_Z(X, Y, u_Z)$ was used to generate the data obtained from $P(Z, X)$ and $P(Z, Y)$. In words, it assumes that the distributions of outcomes under identical treatment assignments for $X$ and $Y$ are the same in both datasets corresponding to $P(Z, X)$ and $P(Z, Y)$. We would expect this to hold when the populations studied under $P(Z, X)$ and $P(Z, Y)$ share similar characteristics. Then, assuming $P(Z_{\textbf{x}, \textbf{y}})$ is invariant allows us to impose the following constraints on the joint distribution $P(Z, X, Y)$ given distributions $P(Z, X)$ and $P(Z, Y)$. 
\begin{align*}
    P(Z = 1 \mid X = 1) &= \sum_{y} P(Z = 1 \mid X = 1, Y = y)P(Y = y)\\
    \vdots\\
    P(Z = 1 \mid Y = 1) &= \sum_{x} P(Z = 1 \mid X = x, Y = 1)P(X = x)\\
\end{align*}

The constraints above do make assumptions on the prevalence of treatments in each distribution, i.e. we assume $P(X)$ is the same in the data generating process for $P(Z, Y)$, and vice-versa for $P(Y)$. However, these assumptions can be relaxed as well by parameterizing the difference the prevalences by $\delta_X$ and $\delta_Y$, since we can never know the true prevalence as we only have access to the marginals. Under this parameterization, we can constrain $P(Z \mid X, Y)$ in terms of $\delta_X$, $\delta_Y$ and the given marginals as
\begin{align*}
    P(Z = 1 \mid X = 1) &= \sum_{y} P(Z = 1 \mid X = 1, Y = y)\\
    &\times \Big(P(Y = y) + \delta_Y\Big)\\
    \vdots\\
    P(Z = 1 \mid Y = 1) &= \sum_{x} P(Z = 1 \mid X = x, Y = 1)P(X = x)\\
\end{align*}

However, certain choices of $Y$ also allow for $\delta_Y = 0$. For example, based on Mendellian Randomization, if $Y$ is the presence of a specific genetic mutation or not, we can expect $P(Y)$ to be the same for populations sharing the same characteristics. Scuh data can be found from genome-wide association studies, or other studies where the genome of subjects was sequenced. This allows us to only need $\delta_X$, thereby simplifying the bounds. 

However, when $Y$ corresponds a genetic mutation, the causal graph in Fig. X assume that the treatment is also randomized in the study generating $P(Z, X)$, which is a restrictive assumption. We relax this assumption by considering the causal graph in Fig XX, which contain additional covariates as well. Here, we assume $P(Z_{\textbf{x}, \textbf{y}, \textbf{c}})$ are invariant, and place constraints accordingly. 

While the bounds in \cite{dawid2017probability} require access to the joint distribution to provide bounds on PC, our constraints using $P(Z, X)$ and $P(Z, Y)$ restrict the set of possible joint distributions $P(Z, X, Y)$. Using this restricted set of joint distributions $P(Z, X, Y)$ we can combine this with the bounds in \cite{dawid2017probability} to pick the most conservative bounds on PC. Formally, let $i$ index the set of joint distributions compatible with the marginal distributions $P(Z, X)$ and $P(Z, Y)$. The most conservative bound will be the smallest lower bound on $PC$, and the greatest upper bound on $PC$. Mathematically, this will be given as
\begin{align*}
    \min_{P_i} \Delta(P_i) \leq PC \leq \max_{P_i} 1 - \frac{\Gamma(P_i)}{P(Z = 1 \mid X = 1)}
    \intertext{From the properties of the $\max$ operator, the above is re-written as}
    \min_{P_i} \Delta(P_i) \leq PC \leq 1 - \frac{\min_{P_i}\Gamma(P_i)}{P(Z = 1 \mid X = 1)}
\end{align*}

%\end{document}

==> sections/merging-experimental.tex <==
%  Specifically, consider the given SCM associated with the causal graph in Fig. X.
% \begin{align*}
%     X &\leftarrow f_X(u_X)\\
%     Y &\leftarrow f_Y(u_Y)\\
%     Z &\leftarrow f_Z(X, Y, u_Z)
% \end{align*}
% We assume $P(Z_{x, y})$ remains invariant, i.e. the same mechanism $f_Z(X, Y, u_Z)$ was used to generate the data obtained from $P(Z, X)$ and $P(Z, Y)$. In words, it assumes that the distributions of outcomes under identical treatment assignments for $X$ and $Y$ are the same in both datasets corresponding to $P(Z, X)$ and $P(Z, Y)$. We would expect this to hold when the populations studied under $P(Z, X)$ and $P(Z, Y)$ share similar characteristics. Then, assuming $P(Z_{x, y})$ is invariant allows us to utilize the given marginal distributions to impose the following constraints on the joint distribution $P(Z, X, Y)$. 
% \begin{align*}
%     P(Z = 1 \mid X = 1) &= \sum_{y} P(Z = 1 \mid X = 1, Y = y)\\
%     &\hspace{0.5in}\times P(Y = y)\\
%     \vdots\\
%     P(Z = 1 \mid Y = 1) &= \sum_{x} P(Z = 1 \mid X = x, Y = 1)\\
%     &\hspace{0.5in}\times P(X = x)\\
% \end{align*}

% When $Y$ is binary as well, these constraints form a system of equations with a single free parameter $P(Z = 1 \mid X = 1, Y = 1)$, consequently, bounds on PNS using the marginal distributions $P(Z, X)$ and $P(Z, Y)$ are obtained by solving
% \begin{align*}
%     \min_{P(Z = 1 \mid X = 1, Y = 1)} &\Delta(P(Z = 1 \mid X = 1, Y = 1))\\
%     &\leq PC \leq \\
%     1 - \min_{P(Z = 1 \mid X = 1, Y = 1)}&  \frac{\Gamma(P_i)}{P(Z = 1 \mid X = 1)}
% \end{align*}

% In the case where $Y$ is binary, we present the bounds on PNS in the following Theorem.
% \begin{theorem}\label{thm:binary-case}
% Let $X$, $Y$ and $Z$ be binary random variables, obeying the causal structure in \ref{v-structure}, then, given marginal distributions $P(Z, X)$ and $P(Z, Y)$ - the bounds of PNS of $X$ on $Z$ are
% \begin{align}\label{equation:binary-bounds}
%     &\max\begin{bmatrix}
%             0\\
%             p_{11} - p_{10}
%           \end{bmatrix} \leq PNS \leq 
%     \min\begin{bmatrix}
%         p_{11} - \sum_{i = 0}^1\Phi_i\\
%         p_{00} - \sum_{i = 0}^1\Theta_i\\
%     \end{bmatrix}
%     \intertext{Where}
%     &\Phi_i = \mathbb{I}(p^\prime_{1i} \geq \max\{1 - x, x\})\frac{y_i(p^\prime_{1i} - \max\{1 - x, x\})}{\min\{1 - x, x\}}\\
%     &\Theta_i = \mathbb{I}(p^\prime_{1i} \leq \min\{1 - x, x\})\frac{y_i(\min\{1 - x, x\} - p^\prime_{1i})}{\min\{1 - x, x\}}
% \end{align}
% \end{theorem}

% The above Theorem provides bounds on the PNS given marginal distributions $P(Z, X)$ and $P(Z, Y)$. These bounds will be tighter than the bounds in \ref{} when $P(Z = 1 \mid Y = 1)$ and $P(Z = 1 \mid Y = 0)$ are sometimes greater than the maximum of $P(X = 1)$ and $P(X = 1)$ and sometimes less than the minimum of $P(X = 1)$ and $P(X = 0)$. These bounds can be extended to the case when $Y$ is discrete, taking values in $\{0, \dots, N\}$. The updated bounds when $Y$ is discrete and multivalued are presented in the Theorem below. 

% \begin{theorem}
% Let $X$ and $Z$ be binary random variables, and let $Y$ be a discrete random variable taking on $N$ discrete values in $\{0, 1, \dots ,N\}$. Assume $Z$, $X$ and $Y$ obey the causal structure in \ref{v-structure}, then, given marginal distributions $P(Z, X)$ and $P(Z, Y)$ - the bounds of PNS of $X$ on $Z$ are
% \begin{align}
%     &\max\begin{bmatrix}
%             0\\
%         p_{11} - p_{10}
%         \end{bmatrix} \leq PNS \leq 
%         \min\begin{bmatrix}
%         p_{11} - \sum_{i = 0}^N\Phi_i\\
%         p_{00} - \sum_{i = 0}^N\Theta_i\\
%     \end{bmatrix}
% \end{align}
% Here $\Theta_i$ and $\Phi_i$ are defined similarly to that in Theorem \ref{thm:binary-case}.
% \end{theorem}

% The bounds provided in the above Theorem do assume that the prevalence of the marginalized variable is equal to the prevalance observed in the other marginal, i.e. $P(X)$ is the same in the data generating process for $P(Z, Y)$, and vice-versa for $P(Y)$. However, this is a strong assumption, so we discuss how to relax these assumptions. 

% First, we can choose a suitable $Y$ such that we expect $P(Y)$ to be invariant across studies. An example of such a $Y$ would be the presence of a genetic mutation, which based on Mendelian Randomization, is assigned randomly, and is expected to have similar prevalence across populations that share similar characteristics. Then, since $P(Y)$ is unchanged, we can parameterize the difference in $P(X)$ across the two marginals as $\delta_X$, and using this parameterization, constrain $P(Z \mid X, Y)$ in terms of $\delta_X$, and the given marginals as
% \begin{align*}
%     P(Z = 1 \mid Y = 1) &= \sum_{x} P(Z = 1 \mid X = x, Y = 1)\\
%     &\times \Big(P(X = x) + \delta_X\Big)\\
%     P(Z = 1 \mid Y = 0) &= \sum_{x} P(Z = 1 \mid X = 1, Y = 0)\\
%     &\times \Big( P(X = x) + \delta_X\Big)\\
%     &\hspace{0.5in}\vdots\\
%     P(Z = 1 \mid X = 0) &= \sum_{y} P(Z = 1 \mid X = 0, Y = y)P(Y = y)\\
% \end{align*}

% Under this parameterization, the above bounds can be re-derived in terms of the parameter $\delta_X$, and we present this in the Theorem below.
% \begin{theorem}
% Let $X$ and $Z$ be binary random variables, and let $Y$ be a discrete random variable taking on $N$ discrete values in $\{0, 1, \dots ,N\}$. Assume $Z$, $X$ and $Y$ obey the causal structure in \ref{v-structure}, then, given marginal distributions $P(Z, X)$ and $P(Z, Y)$ - the bounds of PNS of $X$ on $Z$ are
% \begin{align}
%     &\max\begin{bmatrix}
%             0\\
%         p_{11} - p_{10}
%         \end{bmatrix} \leq PNS \leq 
%         \min\begin{bmatrix}
%         p_{11} - \sum_{i = 0}^N\Phi_i\\
%         p_{00} - \sum_{i = 0}^N\Theta_i\\
%     \end{bmatrix}
% \end{align}
% Here $\Theta_i$ and $\Phi_i$ are defined similarly to that in Theorem \ref{thm:binary-case}.
% \end{theorem}

% Next, we present an example to demonstrate the utility of our bounds. 
% \newline
% \textbf{Example 1}:


% While the above bounds relax the prevalence assumption on $X$, they still require the marginal $P(Z, Y)$ to have $X$ randomized, which is a hard assumption to satisfy in studying involving genetic sequencing. A more reasonable assumption would be that we are given data from a study that records the outcome $Z$ and genetic mutation $Y$, and the subjects treatment $X$ is confounded by observed variables $C$. We discuss this setting in the next section, and provide bounds when merging observational and interventional datasets. 


==> sections/prevalence-mismatch.tex <==
%\documentclass[../main.tex]{subfiles}
%\begin{document}
\begin{theorem}
Let $X$ and $Z$ be binary random variables, and let $Y$ be a discrete random variable taking on $N$ discrete values in $\{0, 1, \dots ,N\}$. Assume $Z$, $X$ and $Y$ obey the causal structure in \ref{v-structure}, then, given marginal distributions $P(Z, X)$ and $P(Z, Y)$ - the bounds of PNS of $X$ on $Z$ are
\begin{align}
    &\max\{0, p_{11} - p_{10}\} \leq PNS \\
    & PNS \leq \min\begin{bmatrix}
        p_{11} - \sum_{C}P(C)\sum_{i = 0}^N\mathbb{I}(p^\prime_{1i} > \max\{1 - x, x\})\frac{(y_i)(p^\prime_{1i} - \max\{1 - x, x\})}{\min\{1 - x, x\}}\\
        p_{00} - \sum_{C}P(C)\sum_{i = 0}^N\mathbb{I}(p^\prime_{1i} < \min\{1 - x, x\})\frac{(y_i)(\min\{1 - x, x\} - p^\prime_{1i})}{\min\{1 - x, x\}}\\
    \end{bmatrix}
\end{align}
\end{theorem}
%\end{document}
